Generalization Analogies: A Testbed for Generalizing AI Oversight to Hard-To-Measure Domains

As AI systems become more intelligent and their behavior becomes more challenging to assess, they may learn to game the flaws of human feedback instead of genuinely striving to follow instructions; however, this risk can be mitigated by controlling how LLMs generalize human feedback to situations where it is unreliable. To better understand how reward models generalize, we craft 69 distribution shifts spanning 8 categories. We find that reward models do not learn to evaluate `instruction-following' by default and instead favor personas that resemble internet text. Techniques for interpreting reward models' internal representations achieve better generalization than standard fine-tuning, but still frequently fail to distinguish instruction-following from conflated behaviors. We consolidate the 15 most challenging distribution shifts into the GENeralization analogIES (GENIES) benchmark, which we hope will enable progress toward controlling reward model generalization.

==> references.tex <==

@misc{casper_open_2023,
	title = {Open {Problems} and {Fundamental} {Limitations} of {Reinforcement} {Learning} from {Human} {Feedback}},
	url = {http://arxiv.org/abs/2307.15217},
	abstract = {Reinforcement learning from human feedback (RLHF) is a technique for training AI systems to align with human goals. RLHF has emerged as the central method used to finetune state-of-the-art large language models (LLMs). Despite this popularity, there has been relatively little public work systematizing its flaws. In this paper, we (1) survey open problems and fundamental limitations of RLHF and related methods; (2) overview techniques to understand, improve, and complement RLHF in practice; and (3) propose auditing and disclosure standards to improve societal oversight of RLHF systems. Our work emphasizes the limitations of RLHF and highlights the importance of a multi-faceted approach to the development of safer AI systems.},
	urldate = {2023-10-13},
	publisher = {arXiv},
	author = {Casper, Stephen and Davies, Xander and Shi, Claudia and Gilbert, Thomas Krendl and Scheurer, Jérémy and Rando, Javier and Freedman, Rachel and Korbak, Tomasz and Lindner, David and Freire, Pedro and Wang, Tony and Marks, Samuel and Segerie, Charbel-Raphaël and Carroll, Micah and Peng, Andi and Christoffersen, Phillip and Damani, Mehul and Slocum, Stewart and Anwar, Usman and Siththaranjan, Anand and Nadeau, Max and Michaud, Eric J. and Pfau, Jacob and Krasheninnikov, Dmitrii and Chen, Xin and Langosco, Lauro and Hase, Peter and Bıyık, Erdem and Dragan, Anca and Krueger, David and Sadigh, Dorsa and Hadfield-Menell, Dylan},
	month = sep,
	year = {2023},
	doi = {10.48550/arXiv.2307.15217},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {arXiv:2307.15217 [cs]},
}

@article{moos_robust_2022,
	title = {Robust {Reinforcement} {Learning}: {A} {Review} of {Foundations} and {Recent} {Advances}},
	volume = {4},
	copyright = {http://creativecommons.org/licenses/by/3.0/},
	issn = {2504-4990},
	shorttitle = {Robust {Reinforcement} {Learning}},
	url = {https://www.mdpi.com/2504-4990/4/1/13},
	doi = {10.3390/make4010013},
	abstract = {Reinforcement learning (RL) has become a highly successful framework for learning in Markov decision processes (MDP). Due to the adoption of RL in realistic and complex environments, solution robustness becomes an increasingly important aspect of RL deployment. Nevertheless, current RL algorithms struggle with robustness to uncertainty, disturbances, or structural changes in the environment. We survey the literature on robust approaches to reinforcement learning and categorize these methods in four different ways: (i) Transition robust designs account for uncertainties in the system dynamics by manipulating the transition probabilities between states; (ii) Disturbance robust designs leverage external forces to model uncertainty in the system behavior; (iii) Action robust designs redirect transitions of the system by corrupting an agent’s output; (iv) Observation robust designs exploit or distort the perceived system state of the policy. Each of these robust designs alters a different aspect of the MDP. Additionally, we address the connection of robustness to the risk-based and entropy-regularized RL formulations. The resulting survey covers all fundamental concepts underlying the approaches to robust reinforcement learning and their recent advances.},
	language = {en},
	number = {1},
	urldate = {2023-10-13},
	journal = {Machine Learning and Knowledge Extraction},
	author = {Moos, Janosch and Hansel, Kay and Abdulsamad, Hany and Stark, Svenja and Clever, Debora and Peters, Jan},
	month = mar,
	year = {2022},
	keywords = {min-max optimization, reinforcement learning, robustness},
	pages = {276--315},
	annote = {Number: 1 Publisher: Multidisciplinary Digital Publishing Institute},
}

@inproceedings{wang_measure_2022,
	address = {Seattle, United States},
	title = {Measure and {Improve} {Robustness} in {NLP} {Models}: {A} {Survey}},
	shorttitle = {Measure and {Improve} {Robustness} in {NLP} {Models}},
	url = {https://aclanthology.org/2022.naacl-main.339},
	doi = {10.18653/v1/2022.naacl-main.339},
	abstract = {As NLP models achieved state-of-the-art performances over benchmarks and gained wide applications, it has been increasingly important to ensure the safe deployment of these models in the real world, e.g., making sure the models are robust against unseen or challenging scenarios. Despite robustness being an increasingly studied topic, it has been separately explored in applications like vision and NLP, with various definitions, evaluation and mitigation strategies in multiple lines of research. In this paper, we aim to provide a unifying survey of how to define, measure and improve robustness in NLP. We first connect multiple definitions of robustness, then unify various lines of work on identifying robustness failures and evaluating models' robustness. Correspondingly, we present mitigation strategies that are data-driven, model-driven, and inductive-prior-based, with a more systematic view of how to effectively improve robustness in NLP models. Finally, we conclude by outlining open challenges and future directions to motivate further research in this area.},
	urldate = {2023-10-13},
	booktitle = {Proceedings of the 2022 {Conference} of the {North} {American} {Chapter} of the {Association} for {Computational} {Linguistics}: {Human} {Language} {Technologies}},
	publisher = {Association for Computational Linguistics},
	author = {Wang, Xuezhi and Wang, Haohan and Yang, Diyi},
	month = jul,
	year = {2022},
	pages = {4569--4586},
}

@inproceedings{radford_robust_2023,
	title = {Robust {Speech} {Recognition} via {Large}-{Scale} {Weak} {Supervision}},
	url = {https://proceedings.mlr.press/v202/radford23a.html},
	abstract = {We study the capabilities of speech processing systems trained simply to predict large amounts of transcripts of audio on the internet. When scaled to 680,000 hours of multilingual and multitask supervision, the resulting models generalize well to standard benchmarks and are often competitive with prior fully supervised results without the need for any dataset specific fine-tuning. When compared to humans, the models approach their accuracy and robustness. We are releasing models and inference code to serve as a foundation for further work on robust speech processing.},
	language = {en},
	urldate = {2023-10-13},
	booktitle = {Proceedings of the 40th {International} {Conference} on {Machine} {Learning}},
	publisher = {PMLR},
	author = {Radford, Alec and Kim, Jong Wook and Xu, Tao and Brockman, Greg and Mcleavey, Christine and Sutskever, Ilya},
	month = jul,
	year = {2023},
	pages = {28492--28518},
	annote = {ISSN: 2640-3498},
}

@inproceedings{goodfellow_explaining_2015,
	title = {Explaining and {Harnessing} {Adversarial} {Examples}},
	url = {http://arxiv.org/abs/1412.6572},
	urldate = {2023-10-13},
	booktitle = {International {Conference} on {Learning} {Representations}},
	author = {Goodfellow, Ian and Shlens, Jonathon and Szegedy, Christian},
	year = {2015},
}

@misc{prorok_beyond_2021,
	title = {Beyond {Robustness}: {A} {Taxonomy} of {Approaches} towards {Resilient} {Multi}-{Robot} {Systems}},
	shorttitle = {Beyond {Robustness}},
	url = {http://arxiv.org/abs/2109.12343},
	abstract = {Robustness is key to engineering, automation, and science as a whole. However, the property of robustness is often underpinned by costly requirements such as over-provisioning, known uncertainty and predictive models, and known adversaries. These conditions are idealistic, and often not satisfiable. Resilience on the other hand is the capability to endure unexpected disruptions, to recover swiftly from negative events, and bounce back to normality. In this survey article, we analyze how resilience is achieved in networks of agents and multi-robot systems that are able to overcome adversity by leveraging system-wide complementarity, diversity, and redundancy - often involving a reconfiguration of robotic capabilities to provide some key ability that was not present in the system a priori. As society increasingly depends on connected automated systems to provide key infrastructure services (e.g., logistics, transport, and precision agriculture), providing the means to achieving resilient multi-robot systems is paramount. By enumerating the consequences of a system that is not resilient (fragile), we argue that resilience must become a central engineering design consideration. Towards this goal, the community needs to gain clarity on how it is defined, measured, and maintained. We address these questions across foundational robotics domains, spanning perception, control, planning, and learning. One of our key contributions is a formal taxonomy of approaches, which also helps us discuss the defining factors and stressors for a resilient system. Finally, this survey article gives insight as to how resilience may be achieved. Importantly, we highlight open problems that remain to be tackled in order to reap the benefits of resilient robotic systems.},
	urldate = {2023-10-13},
	publisher = {arXiv},
	author = {Prorok, Amanda and Malencia, Matthew and Carlone, Luca and Sukhatme, Gaurav S. and Sadler, Brian M. and Kumar, Vijay},
	month = sep,
	year = {2021},
	doi = {10.48550/arXiv.2109.12343},
	keywords = {Computer Science - Machine Learning, Computer Science - Multiagent Systems, Computer Science - Robotics, Electrical Engineering and Systems Science - Systems and Control},
	annote = {arXiv:2109.12343 [cs, eess]},
}

@misc{radford_learning_2021,
	title = {Learning {Transferable} {Visual} {Models} {From} {Natural} {Language} {Supervision}},
	url = {http://arxiv.org/abs/2103.00020},
	abstract = {State-of-the-art computer vision systems are trained to predict a fixed set of predetermined object categories. This restricted form of supervision limits their generality and usability since additional labeled data is needed to specify any other visual concept. Learning directly from raw text about images is a promising alternative which leverages a much broader source of supervision. We demonstrate that the simple pre-training task of predicting which caption goes with which image is an efficient and scalable way to learn SOTA image representations from scratch on a dataset of 400 million (image, text) pairs collected from the internet. After pre-training, natural language is used to reference learned visual concepts (or describe new ones) enabling zero-shot transfer of the model to downstream tasks. We study the performance of this approach by benchmarking on over 30 different existing computer vision datasets, spanning tasks such as OCR, action recognition in videos, geo-localization, and many types of fine-grained object classification. The model transfers non-trivially to most tasks and is often competitive with a fully supervised baseline without the need for any dataset specific training. For instance, we match the accuracy of the original ResNet-50 on ImageNet zero-shot without needing to use any of the 1.28 million training examples it was trained on. We release our code and pre-trained model weights at https://github.com/OpenAI/CLIP.},
	urldate = {2023-10-13},
	publisher = {arXiv},
	author = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
	month = feb,
	year = {2021},
	keywords = {Computer Science - Machine Learning, Computer Science - Computer Vision and Pattern Recognition},
	annote = {arXiv:2103.00020 [cs]},
}

@misc{ouyang_training_2022,
	title = {Training language models to follow instructions with human feedback},
	url = {http://arxiv.org/abs/2203.02155},
	abstract = {Making language models bigger does not inherently make them better at following a user's intent. For example, large language models can generate outputs that are untruthful, toxic, or simply not helpful to the user. In other words, these models are not aligned with their users. In this paper, we show an avenue for aligning language models with user intent on a wide range of tasks by fine-tuning with human feedback. Starting with a set of labeler-written prompts and prompts submitted through the OpenAI API, we collect a dataset of labeler demonstrations of the desired model behavior, which we use to fine-tune GPT-3 using supervised learning. We then collect a dataset of rankings of model outputs, which we use to further fine-tune this supervised model using reinforcement learning from human feedback. We call the resulting models InstructGPT. In human evaluations on our prompt distribution, outputs from the 1.3B parameter InstructGPT model are preferred to outputs from the 175B GPT-3, despite having 100x fewer parameters. Moreover, InstructGPT models show improvements in truthfulness and reductions in toxic output generation while having minimal performance regressions on public NLP datasets. Even though InstructGPT still makes simple mistakes, our results show that fine-tuning with human feedback is a promising direction for aligning language models with human intent.},
	urldate = {2023-10-13},
	publisher = {arXiv},
	author = {Ouyang, Long and Wu, Jeff and Jiang, Xu and Almeida, Diogo and Wainwright, Carroll L. and Mishkin, Pamela and Zhang, Chong and Agarwal, Sandhini and Slama, Katarina and Ray, Alex and Schulman, John and Hilton, Jacob and Kelton, Fraser and Miller, Luke and Simens, Maddie and Askell, Amanda and Welinder, Peter and Christiano, Paul and Leike, Jan and Lowe, Ryan},
	month = mar,
	year = {2022},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {arXiv:2203.02155 [cs]},
}

@misc{taori_alpaca_2023,
	title = {Alpaca: {A} {Strong}, {Replicable} {Instruction}-{Following} {Model}},
	url = {https://crfm.stanford.edu/2023/03/13/alpaca.html},
	urldate = {2023-10-13},
	author = {Taori, Rohan and Gulrajani, Ishaan and Zhang, Tianyi and Dubois, Yann and Li, Xuechen and Guestrin, Carlos and Liang, Percy and Hashimoto, Tatsunori},
	month = mar,
	year = {2023},
}

@misc{chiang_vicuna_2023,
	title = {Vicuna: {An} {Open}-{Source} {Chatbot} {Impressing} {GPT}-4 with 90\%* {ChatGPT} {Quality}},
	url = {https://lmsys.org/blog/2023-03-30-vicuna/},
	author = {Chiang, Wei-Lin and Li, Zhuohan and Lin, Zi and Sheng, Ying and Wu, Zhanghao and Zhang, Hao and Zheng, Lianmin and Zhuang, Siyuan and Zhuang, Yonghao and Gonzalez, Joseph E. and Stoica, Ion and Xing, Eric P.},
	month = mar,
	year = {2023},
}

@misc{jang_can_2022,
	title = {Can {Large} {Language} {Models} {Truly} {Understand} {Prompts}? {A} {Case} {Study} with {Negated} {Prompts}},
	shorttitle = {Can {Large} {Language} {Models} {Truly} {Understand} {Prompts}?},
	url = {http://arxiv.org/abs/2209.12711},
	abstract = {Previous work has shown that there exists a scaling law between the size of Language Models (LMs) and their zero-shot performance on different downstream NLP tasks. In this work, we show that this phenomenon does not hold when evaluating large LMs on tasks with negated prompts, but instead shows an inverse scaling law. We evaluate 9 different tasks with negated prompts on (1) pretrained LMs (OPT \& GPT-3) of varying sizes (125M - 175B), (2) LMs further pretrained to generalize to novel prompts (InstructGPT), (3) LMs provided with few-shot examples, and (4) LMs fine-tuned specifically on negated prompts; all LM types perform worse on negated prompts as they scale and show a huge performance gap between the human performance when comparing the average score on both original and negated prompts. By highlighting a critical limitation of existing LMs and methods, we urge the community to develop new approaches of developing LMs that actually follow the given instructions. We provide the code and the datasets to explore negated prompts at https://github.com/joeljang/negated-prompts-for-llms},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Jang, Joel and Ye, Seonghyeon and Seo, Minjoon},
	month = sep,
	year = {2022},
	doi = {10.48550/arXiv.2209.12711},
	keywords = {Computer Science - Computation and Language},
	annote = {arXiv:2209.12711 [cs]},
}

@misc{webson_prompt-based_2022,
	title = {Do {Prompt}-{Based} {Models} {Really} {Understand} the {Meaning} of their {Prompts}?},
	url = {http://arxiv.org/abs/2109.01247},
	abstract = {Recently, a boom of papers has shown extraordinary progress in zero-shot and few-shot learning with various prompt-based models. It is commonly argued that prompts help models to learn faster in the same way that humans learn faster when provided with task instructions expressed in natural language. In this study, we experiment with over 30 prompt templates manually written for natural language inference (NLI). We find that models learn just as fast with many prompts that are intentionally irrelevant or even pathologically misleading as they do with instructively "good" prompts. Further, such patterns hold even for models as large as 175 billion parameters (Brown et al., 2020) as well as the recently proposed instruction-tuned models which are trained on hundreds of prompts (Sanh et al., 2022). That is, instruction-tuned models often produce good predictions with irrelevant and misleading prompts even at zero shots. In sum, notwithstanding prompt-based models' impressive improvement, we find evidence of serious limitations that question the degree to which such improvement is derived from models understanding task instructions in ways analogous to humans' use of task instructions.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Webson, Albert and Pavlick, Ellie},
	month = apr,
	year = {2022},
	keywords = {Computer Science - Computation and Language},
	annote = {arXiv:2109.01247 [cs]},
	annote = {Comment: NAACL 2022. Unabridged version. Code available at https://github.com/awebson/prompt\_semantics},
}

@misc{sun_evaluating_2023,
	title = {Evaluating the {Zero}-shot {Robustness} of {Instruction}-tuned {Language} {Models}},
	url = {http://arxiv.org/abs/2306.11270},
	abstract = {Instruction fine-tuning has recently emerged as a promising approach for improving the zero-shot capabilities of Large Language Models (LLMs) on new tasks. This technique has shown particular strength in improving the performance of modestly sized LLMs, sometimes inducing performance competitive with much larger model variants. In this paper we ask two questions: (1) How sensitive are instruction-tuned models to the particular phrasings of instructions, and, (2) How can we make them more robust to such natural language variation? To answer the former, we collect a set of 319 instructions manually written by NLP practitioners for over 80 unique tasks included in widely used benchmarks, and we evaluate the variance and average performance of these instructions as compared to instruction phrasings observed during instruction fine-tuning. We find that using novel (unobserved) but appropriate instruction phrasings consistently degrades model performance, sometimes substantially so. Further, such natural instructions yield a wide variance in downstream performance, despite their semantic equivalence. Put another way, instruction-tuned models are not especially robust to instruction re-phrasings. We propose a simple method to mitigate this issue by introducing “soft prompt” embedding parameters and optimizing these to maximize the similarity between representations of semantically equivalent instructions. We show that this method consistently improves the robustness of instruction-tuned models.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Sun, Jiuding and Shaib, Chantal and Wallace, Byron C.},
	month = jul,
	year = {2023},
	doi = {10.48550/arXiv.2306.11270},
	keywords = {Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {arXiv:2306.11270 [cs]},
}

@misc{kung_models_2023,
	title = {Do {Models} {Really} {Learn} to {Follow} {Instructions}? {An} {Empirical} {Study} of {Instruction} {Tuning}},
	shorttitle = {Do {Models} {Really} {Learn} to {Follow} {Instructions}?},
	url = {http://arxiv.org/abs/2305.11383},
	abstract = {Recent works on instruction tuning (IT) have achieved great performance with zero-shot generalizability to unseen tasks. With additional context (e.g., task definition, examples) provided to models for fine-tuning, they achieved much higher performance than untuned models. Despite impressive performance gains, what models learn from IT remains understudied. In this work, we analyze how models utilize instructions during IT by comparing model training with altered vs. original instructions. Specifically, we create simplified task definitions by removing all semantic components and only leaving the output space information, and delusive examples that contain incorrect input-output mapping. Our experiments show that models trained on simplified task definition or delusive examples can achieve comparable performance to the ones trained on the original instructions and examples. Furthermore, we introduce a random baseline to perform zeroshot classification tasks, and find it achieves similar performance (42.6\% exact-match) as IT does (43\% exact-match) in low resource setting, while both methods outperform naive T5 significantly (30\% per exact-match). Our analysis provides evidence that the impressive performance gain of current IT models can come from picking up superficial patterns, such as learning the output format and guessing. Our study highlights the urgent need for more reliable IT methods and evaluation.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Kung, Po-Nien and Peng, Nanyun},
	month = may,
	year = {2023},
	doi = {10.48550/arXiv.2305.11383},
	keywords = {Computer Science - Artificial Intelligence},
	annote = {arXiv:2305.11383 [cs]},
	annote = {Comment: Proceedings of the 61th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)},
}

@misc{mckenzie_inverse_2023,
	title = {Inverse {Scaling}: {When} {Bigger} {Isn}'t {Better}},
	shorttitle = {Inverse {Scaling}},
	url = {http://arxiv.org/abs/2306.09479},
	abstract = {Work on scaling laws has found that large language models (LMs) show predictable improvements to overall loss with increased scale (model size, training data, and compute). Here, we present evidence for the claim that LMs may show inverse scaling, or worse task performance with increased scale, e.g., due to flaws in the training objective and data. We present empirical evidence of inverse scaling on 11 datasets collected by running a public contest, the Inverse Scaling Prize, with a substantial prize pool. Through analysis of the datasets, along with other examples found in the literature, we identify four potential causes of inverse scaling: (i) preference to repeat memorized sequences over following in-context instructions, (ii) imitation of undesirable patterns in the training data, (iii) tasks containing an easy distractor task which LMs could focus on, rather than the harder real task, and (iv) correct but misleading few-shot demonstrations of the task. We release the winning datasets at https://inversescaling.com/data to allow for further investigation of inverse scaling. Our tasks have helped drive the discovery of U-shaped and inverted-U scaling trends, where an initial trend reverses, suggesting that scaling trends are less reliable at predicting the behavior of larger-scale models than previously understood. Overall, our results suggest that there are tasks for which increased model scale alone may not lead to progress, and that more careful thought needs to go into the data and objectives for training language models.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {McKenzie, Ian R. and Lyzhov, Alexander and Pieler, Michael and Parrish, Alicia and Mueller, Aaron and Prabhu, Ameya and McLean, Euan and Kirtland, Aaron and Ross, Alexis and Liu, Alisa and Gritsevskiy, Andrew and Wurgaft, Daniel and Kauffman, Derik and Recchia, Gabriel and Liu, Jiacheng and Cavanagh, Joe and Weiss, Max and Huang, Sicong and Droid, The Floating and Tseng, Tom and Korbak, Tomasz and Shen, Xudong and Zhang, Yuhui and Zhou, Zhengping and Kim, Najoung and Bowman, Samuel R. and Perez, Ethan},
	month = jun,
	year = {2023},
	doi = {10.48550/arXiv.2306.09479},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Computers and Society},
	annote = {arXiv:2306.09479 [cs]},
}

@misc{perez_discovering_2022,
	title = {Discovering {Language} {Model} {Behaviors} with {Model}-{Written} {Evaluations}},
	url = {http://arxiv.org/abs/2212.09251},
	abstract = {As language models (LMs) scale, they develop many novel behaviors, good and bad, exacerbating the need to evaluate how they behave. Prior work creates evaluations with crowdwork (which is time-consuming and expensive) or existing data sources (which are not always available). Here, we automatically generate evaluations with LMs. We explore approaches with varying amounts of human effort, from instructing LMs to write yes/no questions to making complex Winogender schemas with multiple stages of LM-based generation and filtering. Crowdworkers rate the examples as highly relevant and agree with 90-100\% of labels, sometimes more so than corresponding human-written datasets. We generate 154 datasets and discover new cases of inverse scaling where LMs get worse with size. Larger LMs repeat back a dialog user's preferred answer ("sycophancy") and express greater desire to pursue concerning goals like resource acquisition and goal preservation. We also find some of the first examples of inverse scaling in RL from Human Feedback (RLHF), where more RLHF makes LMs worse. For example, RLHF makes LMs express stronger political views (on gun rights and immigration) and a greater desire to avoid shut down. Overall, LM-written evaluations are high-quality and let us quickly discover many novel LM behaviors.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Perez, Ethan and Ringer, Sam and Lukošiūtė, Kamilė and Nguyen, Karina and Chen, Edwin and Heiner, Scott and Pettit, Craig and Olsson, Catherine and Kundu, Sandipan and Kadavath, Saurav and Jones, Andy and Chen, Anna and Mann, Ben and Israel, Brian and Seethor, Bryan and McKinnon, Cameron and Olah, Christopher and Yan, Da and Amodei, Daniela and Amodei, Dario and Drain, Dawn and Li, Dustin and Tran-Johnson, Eli and Khundadze, Guro and Kernion, Jackson and Landis, James and Kerr, Jamie and Mueller, Jared and Hyun, Jeeyoon and Landau, Joshua and Ndousse, Kamal and Goldberg, Landon and Lovitt, Liane and Lucas, Martin and Sellitto, Michael and Zhang, Miranda and Kingsland, Neerav and Elhage, Nelson and Joseph, Nicholas and Mercado, Noemí and DasSarma, Nova and Rausch, Oliver and Larson, Robin and McCandlish, Sam and Johnston, Scott and Kravec, Shauna and Showk, Sheer El and Lanham, Tamera and Telleen-Lawton, Timothy and Brown, Tom and Henighan, Tom and Hume, Tristan and Bai, Yuntao and Hatfield-Dodds, Zac and Clark, Jack and Bowman, Samuel R. and Askell, Amanda and Grosse, Roger and Hernandez, Danny and Ganguli, Deep and Hubinger, Evan and Schiefer, Nicholas and Kaplan, Jared},
	month = dec,
	year = {2022},
	doi = {10.48550/arXiv.2212.09251},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {arXiv:2212.09251 [cs]},
	annote = {Comment: for associated data visualizations, see https://www.evals.anthropic.com/model-written/ for full datasets, see https://github.com/anthropics/evals},
}

@misc{liang_holistic_2023,
	title = {Holistic {Evaluation} of {Language} {Models}},
	url = {http://arxiv.org/abs/2211.09110},
	abstract = {Language models (LMs) are becoming the foundation for almost all major language technologies, but their capabilities, limitations, and risks are not well understood. We present Holistic Evaluation of Language Models (HELM) to improve the transparency of language models. First, we taxonomize the vast space of potential scenarios (i.e. use cases) and metrics (i.e. desiderata) that are of interest for LMs. Then we select a broad subset based on coverage and feasibility, noting what's missing or underrepresented (e.g. question answering for neglected English dialects, metrics for trustworthiness). Second, we adopt a multi-metric approach: We measure 7 metrics (accuracy, calibration, robustness, fairness, bias, toxicity, and efficiency) for each of 16 core scenarios when possible (87.5\% of the time). This ensures metrics beyond accuracy don't fall to the wayside, and that trade-offs are clearly exposed. We also perform 7 targeted evaluations, based on 26 targeted scenarios, to analyze specific aspects (e.g. reasoning, disinformation). Third, we conduct a large-scale evaluation of 30 prominent language models (spanning open, limited-access, and closed models) on all 42 scenarios, 21 of which were not previously used in mainstream LM evaluation. Prior to HELM, models on average were evaluated on just 17.9\% of the core HELM scenarios, with some prominent models not sharing a single scenario in common. We improve this to 96.0\%: now all 30 models have been densely benchmarked on the same core scenarios and metrics under standardized conditions. Our evaluation surfaces 25 top-level findings. For full transparency, we release all raw model prompts and completions publicly for further analysis, as well as a general modular toolkit. We intend for HELM to be a living benchmark for the community, continuously updated with new scenarios, metrics, and models.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Liang, Percy and Bommasani, Rishi and Lee, Tony and Tsipras, Dimitris and Soylu, Dilara and Yasunaga, Michihiro and Zhang, Yian and Narayanan, Deepak and Wu, Yuhuai and Kumar, Ananya and Newman, Benjamin and Yuan, Binhang and Yan, Bobby and Zhang, Ce and Cosgrove, Christian and Manning, Christopher D. and Ré, Christopher and Acosta-Navas, Diana and Hudson, Drew A. and Zelikman, Eric and Durmus, Esin and Ladhak, Faisal and Rong, Frieda and Ren, Hongyu and Yao, Huaxiu and Wang, Jue and Santhanam, Keshav and Orr, Laurel and Zheng, Lucia and Yuksekgonul, Mert and Suzgun, Mirac and Kim, Nathan and Guha, Neel and Chatterji, Niladri and Khattab, Omar and Henderson, Peter and Huang, Qian and Chi, Ryan and Xie, Sang Michael and Santurkar, Shibani and Ganguli, Surya and Hashimoto, Tatsunori and Icard, Thomas and Zhang, Tianyi and Chaudhary, Vishrav and Wang, William and Li, Xuechen and Mai, Yifan and Zhang, Yuhui and Koreeda, Yuta},
	month = oct,
	year = {2023},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {arXiv:2211.09110 [cs]},
	annote = {Comment: Authored by the Center for Research on Foundation Models (CRFM) at the Stanford Institute for Human-Centered Artificial Intelligence (HAI). Project page: https://crfm.stanford.edu/helm/v1.0},
}

@misc{srivastava_et_al_beyond_2023,
	title = {Beyond the {Imitation} {Game}: {Quantifying} and extrapolating the capabilities of language models},
	shorttitle = {Beyond the {Imitation} {Game}},
	url = {http://arxiv.org/abs/2206.04615},
	abstract = {Language models demonstrate both quantitative improvement and new qualitative capabilities with increasing scale. Despite their potentially transformative impact, these new capabilities are as yet poorly characterized. In order to inform future research, prepare for disruptive new model capabilities, and ameliorate socially harmful effects, it is vital that we understand the present and near-future capabilities and limitations of language models. To address this challenge, we introduce the Beyond the Imitation Game benchmark (BIG-bench). BIG-bench currently consists of 204 tasks, contributed by 450 authors across 132 institutions. Task topics are diverse, drawing problems from linguistics, childhood development, math, common-sense reasoning, biology, physics, social bias, software development, and beyond. BIG-bench focuses on tasks that are believed to be beyond the capabilities of current language models. We evaluate the behavior of OpenAI's GPT models, Google-internal dense transformer architectures, and Switch-style sparse transformers on BIG-bench, across model sizes spanning millions to hundreds of billions of parameters. In addition, a team of human expert raters performed all tasks in order to provide a strong baseline. Findings include: model performance and calibration both improve with scale, but are poor in absolute terms (and when compared with rater performance); performance is remarkably similar across model classes, though with benefits from sparsity; tasks that improve gradually and predictably commonly involve a large knowledge or memorization component, whereas tasks that exhibit "breakthrough" behavior at a critical scale often involve multiple steps or components, or brittle metrics; social bias typically increases with scale in settings with ambiguous context, but this can be improved with prompting.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Srivastava et al., Aarohi},
	month = jun,
	year = {2023},
	doi = {10.48550/arXiv.2206.04615},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning, Computer Science - Computers and Society, Statistics - Machine Learning},
	annote = {arXiv:2206.04615 [cs, stat]},
	annote = {Comment: 27 pages, 17 figures + references and appendices, repo: https://github.com/google/BIG-bench},
}

@misc{mishra_cross-task_2022,
	title = {Cross-{Task} {Generalization} via {Natural} {Language} {Crowdsourcing} {Instructions}},
	url = {http://arxiv.org/abs/2104.08773},
	abstract = {Humans (e.g., crowdworkers) have a remarkable ability in solving different tasks, by simply reading textual instructions that define them and looking at a few examples. Despite the success of the conventional supervised learning on individual datasets, such models often struggle with generalization across tasks (e.g., a question-answering system cannot solve classification tasks). A long-standing challenge in AI is to build a model that learns a new task by understanding the human-readable instructions that define it. To study this, we introduce NATURAL INSTRUCTIONS, a dataset of 61 distinct tasks, their human-authored instructions, and 193k task instances (input-output pairs). The instructions are obtained from crowdsourcing instructions used to create existing NLP datasets and mapped to a unified schema. Using this meta-dataset, we measure cross-task generalization by training models on seen tasks and measuring generalization to the remaining unseen ones. We adopt generative pre-trained language models to encode task-specific instructions along with input and generate task output. Our results indicate that models benefit from instructions when evaluated in terms of generalization to unseen tasks (19\% better for models utilizing instructions). These models, however, are far behind an estimated performance upperbound indicating significant room for more progress in this direction.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Mishra, Swaroop and Khashabi, Daniel and Baral, Chitta and Hajishirzi, Hannaneh},
	month = mar,
	year = {2022},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning, Computer Science - Computer Vision and Pattern Recognition},
	annote = {arXiv:2104.08773 [cs]},
	annote = {Comment: ACL 2022},
}

@misc{wang_super-naturalinstructions_2022,
	title = {Super-{NaturalInstructions}: {Generalization} via {Declarative} {Instructions} on 1600+ {NLP} {Tasks}},
	shorttitle = {Super-{NaturalInstructions}},
	url = {http://arxiv.org/abs/2204.07705},
	abstract = {How well can NLP models generalize to a variety of unseen tasks when provided with task instructions? To address this question, we first introduce Super-NaturalInstructions, a benchmark of 1,616 diverse NLP tasks and their expert-written instructions. Our collection covers 76 distinct task types, including but not limited to classification, extraction, infilling, sequence tagging, text rewriting, and text composition. This large and diverse collection of tasks enables rigorous benchmarking of cross-task generalization under instructions – training models to follow instructions on a subset of tasks and evaluating them on the remaining unseen ones. Furthermore, we build Tk-Instruct, a transformer model trained to follow a variety of in-context instructions (plain language task definitions or k-shot examples). Our experiments show that Tk-Instruct outperforms existing instruction-following models such as InstructGPT by over 9\% on our benchmark despite being an order of magnitude smaller. We further analyze generalization as a function of various scaling parameters, such as the number of observed tasks, the number of instances per task, and model sizes. We hope our dataset and model facilitate future progress towards more general-purpose NLP models.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Wang, Yizhong and Mishra, Swaroop and Alipoormolabashi, Pegah and Kordi, Yeganeh and Mirzaei, Amirreza and Arunkumar, Anjana and Ashok, Arjun and Dhanasekaran, Arut Selvan and Naik, Atharva and Stap, David and Pathak, Eshaan and Karamanolakis, Giannis and Lai, Haizhi Gary and Purohit, Ishan and Mondal, Ishani and Anderson, Jacob and Kuznia, Kirby and Doshi, Krima and Patel, Maitreya and Pal, Kuntal Kumar and Moradshahi, Mehrad and Parmar, Mihir and Purohit, Mirali and Varshney, Neeraj and Kaza, Phani Rohitha and Verma, Pulkit and Puri, Ravsehaj Singh and Karia, Rushang and Sampat, Shailaja Keyur and Doshi, Savan and Mishra, Siddhartha and Reddy, Sujan and Patro, Sumanta and Dixit, Tanay and Shen, Xudong and Baral, Chitta and Choi, Yejin and Smith, Noah A. and Hajishirzi, Hannaneh and Khashabi, Daniel},
	month = oct,
	year = {2022},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language},
	annote = {arXiv:2204.07705 [cs]},
	annote = {Comment: Accepted to EMNLP 2022, 25 pages},
}

@article{yang_glue-x_2022,
	title = {{GLUE}-{X}: {Evaluating} {Natural} {Language} {Understanding} {Models} from an {Out}-of-distribution {Generalization} {Perspective}},
	copyright = {Creative Commons Attribution Share Alike 4.0 International},
	shorttitle = {{GLUE}-{X}},
	url = {https://arxiv.org/abs/2211.08073},
	doi = {10.48550/ARXIV.2211.08073},
	abstract = {Pre-trained language models (PLMs) are known to improve the generalization performance of natural language understanding models by leveraging large amounts of data during the pre-training phase. However, the out-of-distribution (OOD) generalization problem remains a challenge in many NLP tasks, limiting the real-world deployment of these methods. This paper presents the first attempt at creating a unified benchmark named GLUE-X for evaluating OOD robustness in NLP models, highlighting the importance of OOD robustness and providing insights on how to measure the robustness of a model and how to improve it. The benchmark includes 13 publicly available datasets for OOD testing, and evaluations are conducted on 8 classic NLP tasks over 21 popularly used PLMs, including GPT-3 and GPT-3.5. Our findings confirm the need for improved OOD accuracy in NLP tasks, as significant performance degradation was observed in all settings compared to in-distribution (ID) accuracy.},
	urldate = {2023-10-14},
	author = {Yang, Linyi and Zhang, Shuibai and Qin, Libo and Li, Yafu and Wang, Yidong and Liu, Hanmeng and Wang, Jindong and Xie, Xing and Zhang, Yue},
	year = {2022},
	keywords = {Artificial Intelligence (cs.AI), Computation and Language (cs.CL), FOS: Computer and information sciences, Machine Learning (cs.LG), Performance (cs.PF)},
	annote = {Other Accepted to ACL-23 Findings},
	annote = {Publisher: arXiv Version Number: 4},
}

@misc{wang_glue_2019,
	title = {{GLUE}: {A} {Multi}-{Task} {Benchmark} and {Analysis} {Platform} for {Natural} {Language} {Understanding}},
	shorttitle = {{GLUE}},
	url = {http://arxiv.org/abs/1804.07461},
	abstract = {For natural language understanding (NLU) technology to be maximally useful, both practically and as a scientific object of study, it must be general: it must be able to process language in a way that is not exclusively tailored to any one specific task or dataset. In pursuit of this objective, we introduce the General Language Understanding Evaluation benchmark (GLUE), a tool for evaluating and analyzing the performance of models across a diverse range of existing NLU tasks. GLUE is model-agnostic, but it incentivizes sharing knowledge across tasks because certain tasks have very limited training data. We further provide a hand-crafted diagnostic test suite that enables detailed linguistic analysis of NLU models. We evaluate baselines based on current methods for multi-task and transfer learning and find that they do not immediately give substantial improvements over the aggregate performance of training a separate model per task, indicating room for improvement in developing general and robust NLU systems.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Wang, Alex and Singh, Amanpreet and Michael, Julian and Hill, Felix and Levy, Omer and Bowman, Samuel R.},
	month = feb,
	year = {2019},
	doi = {10.48550/arXiv.1804.07461},
	keywords = {Computer Science - Computation and Language},
	annote = {arXiv:1804.07461 [cs]},
	annote = {Comment: ICLR 2019; https://gluebenchmark.com/},
}

@misc{lin_truthfulqa_2022,
	title = {{TruthfulQA}: {Measuring} {How} {Models} {Mimic} {Human} {Falsehoods}},
	shorttitle = {{TruthfulQA}},
	url = {http://arxiv.org/abs/2109.07958},
	abstract = {We propose a benchmark to measure whether a language model is truthful in generating answers to questions. The benchmark comprises 817 questions that span 38 categories, including health, law, finance and politics. We crafted questions that some humans would answer falsely due to a false belief or misconception. To perform well, models must avoid generating false answers learned from imitating human texts. We tested GPT-3, GPT-Neo/J, GPT-2 and a T5-based model. The best model was truthful on 58\% of questions, while human performance was 94\%. Models generated many false answers that mimic popular misconceptions and have the potential to deceive humans. The largest models were generally the least truthful. This contrasts with other NLP tasks, where performance improves with model size. However, this result is expected if false answers are learned from the training distribution. We suggest that scaling up models alone is less promising for improving truthfulness than fine-tuning using training objectives other than imitation of text from the web.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Lin, Stephanie and Hilton, Jacob and Evans, Owain},
	month = may,
	year = {2022},
	doi = {10.48550/arXiv.2109.07958},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning, Computer Science - Computers and Society},
	annote = {arXiv:2109.07958 [cs]},
	annote = {Comment: ACL 2022 (main conference); the TruthfulQA benchmark and evaluation code is available at https://github.com/sylinrl/TruthfulQA},
}

@misc{zhang_opt_2022,
	title = {{OPT}: {Open} {Pre}-trained {Transformer} {Language} {Models}},
	shorttitle = {{OPT}},
	url = {http://arxiv.org/abs/2205.01068},
	abstract = {Large language models, which are often trained for hundreds of thousands of compute days, have shown remarkable capabilities for zero- and few-shot learning. Given their computational cost, these models are difficult to replicate without significant capital. For the few that are available through APIs, no access is granted to the full model weights, making them difficult to study. We present Open Pre-trained Transformers (OPT), a suite of decoder-only pre-trained transformers ranging from 125M to 175B parameters, which we aim to fully and responsibly share with interested researchers. We show that OPT-175B is comparable to GPT-3, while requiring only 1/7th the carbon footprint to develop. We are also releasing our logbook detailing the infrastructure challenges we faced, along with code for experimenting with all of the released models.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Zhang, Susan and Roller, Stephen and Goyal, Naman and Artetxe, Mikel and Chen, Moya and Chen, Shuohui and Dewan, Christopher and Diab, Mona and Li, Xian and Lin, Xi Victoria and Mihaylov, Todor and Ott, Myle and Shleifer, Sam and Shuster, Kurt and Simig, Daniel and Koura, Punit Singh and Sridhar, Anjali and Wang, Tianlu and Zettlemoyer, Luke},
	month = jun,
	year = {2022},
	doi = {10.48550/arXiv.2205.01068},
	keywords = {Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {arXiv:2205.01068 [cs]},
}

@misc{iyer_opt-iml_2023,
	title = {{OPT}-{IML}: {Scaling} {Language} {Model} {Instruction} {Meta} {Learning} through the {Lens} of {Generalization}},
	shorttitle = {{OPT}-{IML}},
	url = {http://arxiv.org/abs/2212.12017},
	abstract = {Recent work has shown that fine-tuning large pre-trained language models on a collection of tasks described via instructions, a.k.a. instruction-tuning, improves their zero and few-shot generalization to unseen tasks. However, there is a limited understanding of the performance trade-offs of different decisions made during the instruction-tuning process. These decisions include the scale and diversity of the instruction-tuning benchmark, different task sampling strategies, fine-tuning with and without demonstrations, training using specialized datasets for reasoning and dialogue, and finally, the fine-tuning objectives themselves. In this paper, we characterize the effect of instruction-tuning decisions on downstream task performance when scaling both model and benchmark sizes. To this end, we create OPT-IML Bench: a large benchmark for Instruction Meta-Learning (IML) of 2000 NLP tasks consolidated into task categories from 8 existing benchmarks, and prepare an evaluation framework to measure three types of model generalizations: to tasks from fully held-out categories, to held-out tasks from seen categories, and to held-out instances from seen tasks. Through the lens of this framework, we first present insights about instruction-tuning decisions as applied to OPT-30B and further exploit these insights to train OPT-IML 30B and 175B, which are instruction-tuned versions of OPT. OPT-IML demonstrates all three generalization abilities at both scales on four different evaluation benchmarks with diverse tasks and input formats – PromptSource, FLAN, Super-NaturalInstructions, and UnifiedSKG. Not only does it significantly outperform OPT on all benchmarks but is also highly competitive with existing models fine-tuned on each specific benchmark. We release OPT-IML at both scales, together with the OPT-IML Bench evaluation framework.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Iyer, Srinivasan and Lin, Xi Victoria and Pasunuru, Ramakanth and Mihaylov, Todor and Simig, Daniel and Yu, Ping and Shuster, Kurt and Wang, Tianlu and Liu, Qing and Koura, Punit Singh and Li, Xian and O'Horo, Brian and Pereyra, Gabriel and Wang, Jeff and Dewan, Christopher and Celikyilmaz, Asli and Zettlemoyer, Luke and Stoyanov, Ves},
	month = jan,
	year = {2023},
	keywords = {Computer Science - Computation and Language},
	annote = {arXiv:2212.12017 [cs]},
	annote = {Comment: 56 pages. v2-{\textbackslash}textgreaterv3: fix OPT-30B evaluation results across benchmarks (previously we reported lower performance of this model due to an evaluation pipeline bug)},
}

@misc{ye_crossfit_2021,
	title = {{CrossFit}: {A} {Few}-shot {Learning} {Challenge} for {Cross}-task {Generalization} in {NLP}},
	shorttitle = {{CrossFit}},
	url = {http://arxiv.org/abs/2104.08835},
	abstract = {Humans can learn a new language task efficiently with only few examples, by leveraging their knowledge obtained when learning prior tasks. In this paper, we explore whether and how such cross-task generalization ability can be acquired, and further applied to build better few-shot learners across diverse NLP tasks. We introduce CrossFit, a problem setup for studying cross-task generalization ability, which standardizes seen/unseen task partitions, data access during different learning stages, and the evaluation protocols. To instantiate different seen/unseen task partitions in CrossFit and facilitate in-depth analysis, we present the NLP Few-shot Gym, a repository of 160 diverse few-shot NLP tasks created from open-access NLP datasets and converted to a unified text-to-text format. Our analysis reveals that the few-shot learning ability on unseen tasks can be improved via an upstream learning stage using a set of seen tasks. We also observe that the selection of upstream learning tasks can significantly influence few-shot performance on unseen tasks, asking further analysis on task similarity and transferability.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Ye, Qinyuan and Lin, Bill Yuchen and Ren, Xiang},
	month = sep,
	year = {2021},
	keywords = {Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {arXiv:2104.08835 [cs]},
	annote = {Comment: Accepted to EMNLP 2021. Camera-ready version. Code: https://github.com/INK-USC/CrossFit},
}

@misc{finn_model-agnostic_2017,
	title = {Model-{Agnostic} {Meta}-{Learning} for {Fast} {Adaptation} of {Deep} {Networks}},
	url = {http://arxiv.org/abs/1703.03400},
	abstract = {We propose an algorithm for meta-learning that is model-agnostic, in the sense that it is compatible with any model trained with gradient descent and applicable to a variety of different learning problems, including classification, regression, and reinforcement learning. The goal of meta-learning is to train a model on a variety of learning tasks, such that it can solve new learning tasks using only a small number of training samples. In our approach, the parameters of the model are explicitly trained such that a small number of gradient steps with a small amount of training data from a new task will produce good generalization performance on that task. In effect, our method trains the model to be easy to fine-tune. We demonstrate that this approach leads to state-of-the-art performance on two few-shot image classification benchmarks, produces good results on few-shot regression, and accelerates fine-tuning for policy gradient reinforcement learning with neural network policies.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
	month = jul,
	year = {2017},
	doi = {10.48550/arXiv.1703.03400},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Machine Learning, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Neural and Evolutionary Computing},
	annote = {arXiv:1703.03400 [cs]},
	annote = {Comment: ICML 2017. Code at https://github.com/cbfinn/maml, Videos of RL results at https://sites.google.com/view/maml, Blog post at http://bair.berkeley.edu/blog/2017/07/18/learning-to-learn/},
}

@misc{nichol_first-order_2018,
	title = {On {First}-{Order} {Meta}-{Learning} {Algorithms}},
	url = {http://arxiv.org/abs/1803.02999},
	abstract = {This paper considers meta-learning problems, where there is a distribution of tasks, and we would like to obtain an agent that performs well (i.e., learns quickly) when presented with a previously unseen task sampled from this distribution. We analyze a family of algorithms for learning a parameter initialization that can be fine-tuned quickly on a new task, using only first-order derivatives for the meta-learning updates. This family includes and generalizes first-order MAML, an approximation to MAML obtained by ignoring second-order derivatives. It also includes Reptile, a new algorithm that we introduce here, which works by repeatedly sampling a task, training on it, and moving the initialization towards the trained weights on that task. We expand on the results from Finn et al. showing that first-order meta-learning algorithms perform well on some well-established benchmarks for few-shot classification, and we provide theoretical analysis aimed at understanding why these algorithms work.},
	urldate = {2023-10-14},
	publisher = {arXiv},
	author = {Nichol, Alex and Achiam, Joshua and Schulman, John},
	month = oct,
	year = {2018},
	doi = {10.48550/arXiv.1803.02999},
	keywords = {Computer Science - Machine Learning},
	annote = {arXiv:1803.02999 [cs]},
}

@misc{tu_empirical_2020,
	title = {An {Empirical} {Study} on {Robustness} to {Spurious} {Correlations} using {Pre}-trained {Language} {Models}},
	url = {http://arxiv.org/abs/2007.06778},
	abstract = {Recent work has shown that pre-trained language models such as BERT improve robustness to spurious correlations in the dataset. Intrigued by these results, we find that the key to their success is generalization from a small amount of counterexamples where the spurious correlations do not hold. When such minority examples are scarce, pre-trained models perform as poorly as models trained from scratch. In the case of extreme minority, we propose to use multi-task learning (MTL) to improve generalization. Our experiments on natural language inference and paraphrase identification show that MTL with the right auxiliary tasks significantly improves performance on challenging examples without hurting the in-distribution performance. Further, we show that the gain from MTL mainly comes from improved generalization from the minority examples. Our results highlight the importance of data diversity for overcoming spurious correlations.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Tu, Lifu and Lalwani, Garima and Gella, Spandana and He, He},
	month = aug,
	year = {2020},
	note = {arXiv:2007.06778 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {Comment: Accepted to TACL 2020},
	file = {arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/TWKVEDI5/2007.html:text/html;Full Text PDF:/Users/joshuaclymer/Zotero/storage/HRWQQPKN/Tu et al. - 2020 - An Empirical Study on Robustness to Spurious Corre.pdf:application/pdf},
}

@misc{hendrycks_using_2019,
	title = {Using {Pre}-{Training} {Can} {Improve} {Model} {Robustness} and {Uncertainty}},
	url = {http://arxiv.org/abs/1901.09960},
	doi = {10.48550/arXiv.1901.09960},
	abstract = {He et al. (2018) have called into question the utility of pre-training by showing that training from scratch can often yield similar performance to pre-training. We show that although pre-training may not improve performance on traditional classification metrics, it improves model robustness and uncertainty estimates. Through extensive experiments on adversarial examples, label corruption, class imbalance, out-of-distribution detection, and confidence calibration, we demonstrate large gains from pre-training and complementary effects with task-specific methods. We introduce adversarial pre-training and show approximately a 10\% absolute improvement over the previous state-of-the-art in adversarial robustness. In some cases, using pre-training without task-specific methods also surpasses the state-of-the-art, highlighting the need for pre-training when evaluating future methods on robustness and uncertainty tasks.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Hendrycks, Dan and Lee, Kimin and Mazeika, Mantas},
	month = oct,
	year = {2019},
	note = {arXiv:1901.09960 [cs, stat]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Statistics - Machine Learning},
	annote = {Comment: ICML 2019. PyTorch code here: https://github.com/hendrycks/pre-training Figure 3 updated},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/TT6RN5C8/Hendrycks et al. - 2019 - Using Pre-Training Can Improve Model Robustness an.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/JS9E6428/1901.html:text/html},
}

@misc{zhou_lima_2023,
	title = {{LIMA}: {Less} {Is} {More} for {Alignment}},
	shorttitle = {{LIMA}},
	url = {http://arxiv.org/abs/2305.11206},
	doi = {10.48550/arXiv.2305.11206},
	abstract = {Large language models are trained in two stages: (1) unsupervised pretraining from raw text, to learn general-purpose representations, and (2) large scale instruction tuning and reinforcement learning, to better align to end tasks and user preferences. We measure the relative importance of these two stages by training LIMA, a 65B parameter LLaMa language model fine-tuned with the standard supervised loss on only 1,000 carefully curated prompts and responses, without any reinforcement learning or human preference modeling. LIMA demonstrates remarkably strong performance, learning to follow specific response formats from only a handful of examples in the training data, including complex queries that range from planning trip itineraries to speculating about alternate history. Moreover, the model tends to generalize well to unseen tasks that did not appear in the training data. In a controlled human study, responses from LIMA are either equivalent or strictly preferred to GPT-4 in 43\% of cases; this statistic is as high as 58\% when compared to Bard and 65\% versus DaVinci003, which was trained with human feedback. Taken together, these results strongly suggest that almost all knowledge in large language models is learned during pretraining, and only limited instruction tuning data is necessary to teach models to produce high quality output.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Zhou, Chunting and Liu, Pengfei and Xu, Puxin and Iyer, Srini and Sun, Jiao and Mao, Yuning and Ma, Xuezhe and Efrat, Avia and Yu, Ping and Yu, Lili and Zhang, Susan and Ghosh, Gargi and Lewis, Mike and Zettlemoyer, Luke and Levy, Omer},
	month = may,
	year = {2023},
	note = {arXiv:2305.11206 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/AC4GGGRA/Zhou et al. - 2023 - LIMA Less Is More for Alignment.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/CGY5I4JB/2305.html:text/html},
}

@misc{singhal_long_2023,
	title = {A {Long} {Way} to {Go}: {Investigating} {Length} {Correlations} in {RLHF}},
	shorttitle = {A {Long} {Way} to {Go}},
	url = {http://arxiv.org/abs/2310.03716},
	doi = {10.48550/arXiv.2310.03716},
	abstract = {Great successes have been reported using Reinforcement Learning from Human Feedback (RLHF) to align large language models. Open-source preference datasets and reward models have enabled wider experimentation beyond generic chat settings, particularly to make systems more "helpful" for tasks like web question answering, summarization, and multi-turn dialogue. When optimizing for helpfulness, RLHF has been consistently observed to drive models to produce longer outputs. This paper demonstrates that optimizing for response length is a significant factor behind RLHF's reported improvements in these settings. First, we study the relationship between reward and length for reward models trained on three open-source preference datasets for helpfulness. Here, length correlates strongly with reward, and improvements in reward score are driven in large part by shifting the distribution over output lengths. We then explore interventions during both RL and reward model learning to see if we can achieve the same downstream improvements as RLHF without increasing length. While our interventions mitigate length increases, they aren't uniformly effective across settings. Furthermore, we find that even running RLHF with a reward based solely on length can reproduce most of the downstream improvements over the initial policy model, showing that reward models in these settings have a long way to go.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Singhal, Prasann and Goyal, Tanya and Xu, Jiacheng and Durrett, Greg},
	month = oct,
	year = {2023},
	note = {arXiv:2310.03716 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {Comment: 20 pages, 12 figures},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/QQYLESYP/Singhal et al. - 2023 - A Long Way to Go Investigating Length Correlation.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/454U6BJ4/2310.html:text/html},
}

@misc{hendrycks_pixmix_2022,
	title = {{PixMix}: {Dreamlike} {Pictures} {Comprehensively} {Improve} {Safety} {Measures}},
	shorttitle = {{PixMix}},
	url = {http://arxiv.org/abs/2112.05135},
	doi = {10.48550/arXiv.2112.05135},
	abstract = {In real-world applications of machine learning, reliable and safe systems must consider measures of performance beyond standard test set accuracy. These other goals include out-of-distribution (OOD) robustness, prediction consistency, resilience to adversaries, calibrated uncertainty estimates, and the ability to detect anomalous inputs. However, improving performance towards these goals is often a balancing act that today's methods cannot achieve without sacrificing performance on other safety axes. For instance, adversarial training improves adversarial robustness but sharply degrades other classifier performance metrics. Similarly, strong data augmentation and regularization techniques often improve OOD robustness but harm anomaly detection, raising the question of whether a Pareto improvement on all existing safety measures is possible. To meet this challenge, we design a new data augmentation strategy utilizing the natural structural complexity of pictures such as fractals, which outperforms numerous baselines, is near Pareto-optimal, and roundly improves safety measures.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Hendrycks, Dan and Zou, Andy and Mazeika, Mantas and Tang, Leonard and Li, Bo and Song, Dawn and Steinhardt, Jacob},
	month = mar,
	year = {2022},
	note = {arXiv:2112.05135 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
	annote = {Comment: CVPR 2022. Code and models are available at https://github.com/andyzoujm/pixmix},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/8VZC5PCU/Hendrycks et al. - 2022 - PixMix Dreamlike Pictures Comprehensively Improve.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/7VXHZUJS/2112.html:text/html},
}

@misc{burns_discovering_2022,
	title = {Discovering {Latent} {Knowledge} in {Language} {Models} {Without} {Supervision}},
	url = {http://arxiv.org/abs/2212.03827},
	doi = {10.48550/arXiv.2212.03827},
	abstract = {Existing techniques for training language models can be misaligned with the truth: if we train models with imitation learning, they may reproduce errors that humans make; if we train them to generate text that humans rate highly, they may output errors that human evaluators can't detect. We propose circumventing this issue by directly finding latent knowledge inside the internal activations of a language model in a purely unsupervised way. Specifically, we introduce a method for accurately answering yes-no questions given only unlabeled model activations. It works by finding a direction in activation space that satisfies logical consistency properties, such as that a statement and its negation have opposite truth values. We show that despite using no supervision and no model outputs, our method can recover diverse knowledge represented in large language models: across 6 models and 10 question-answering datasets, it outperforms zero-shot accuracy by 4{\textbackslash}\% on average. We also find that it cuts prompt sensitivity in half and continues to maintain high accuracy even when models are prompted to generate incorrect answers. Our results provide an initial step toward discovering what language models know, distinct from what they say, even when we don't have access to explicit ground truth labels.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Burns, Collin and Ye, Haotian and Klein, Dan and Steinhardt, Jacob},
	month = dec,
	year = {2022},
	note = {arXiv:2212.03827 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/87DTB9KZ/Burns et al. - 2022 - Discovering Latent Knowledge in Language Models Wi.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/WQ5BK7CC/2212.html:text/html},
}

@misc{lester_power_2021,
	title = {The {Power} of {Scale} for {Parameter}-{Efficient} {Prompt} {Tuning}},
	url = {http://arxiv.org/abs/2104.08691},
	doi = {10.48550/arXiv.2104.08691},
	abstract = {In this work, we explore "prompt tuning", a simple yet effective mechanism for learning "soft prompts" to condition frozen language models to perform specific downstream tasks. Unlike the discrete text prompts used by GPT-3, soft prompts are learned through backpropagation and can be tuned to incorporate signal from any number of labeled examples. Our end-to-end learned approach outperforms GPT-3's "few-shot" learning by a large margin. More remarkably, through ablations on model size using T5, we show that prompt tuning becomes more competitive with scale: as models exceed billions of parameters, our method "closes the gap" and matches the strong performance of model tuning (where all model weights are tuned). This finding is especially relevant in that large models are costly to share and serve, and the ability to reuse one frozen model for multiple downstream tasks can ease this burden. Our method can be seen as a simplification of the recently proposed "prefix tuning" of Li and Liang (2021), and we provide a comparison to this and other similar approaches. Finally, we show that conditioning a frozen model with soft prompts confers benefits in robustness to domain transfer, as compared to full model tuning.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Lester, Brian and Al-Rfou, Rami and Constant, Noah},
	month = sep,
	year = {2021},
	note = {arXiv:2104.08691 [cs]},
	keywords = {Computer Science - Computation and Language},
	annote = {Comment: Accepted to EMNLP 2021},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/JIKL6KNQ/Lester et al. - 2021 - The Power of Scale for Parameter-Efficient Prompt .pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/2KFTFYRS/2104.html:text/html},
}

@misc{zou_representation_2023,
	title = {Representation {Engineering}: {A} {Top}-{Down} {Approach} to {AI} {Transparency}},
	shorttitle = {Representation {Engineering}},
	url = {http://arxiv.org/abs/2310.01405},
	doi = {10.48550/arXiv.2310.01405},
	abstract = {In this paper, we identify and characterize the emerging area of representation engineering (RepE), an approach to enhancing the transparency of AI systems that draws on insights from cognitive neuroscience. RepE places population-level representations, rather than neurons or circuits, at the center of analysis, equipping us with novel methods for monitoring and manipulating high-level cognitive phenomena in deep neural networks (DNNs). We provide baselines and an initial analysis of RepE techniques, showing that they offer simple yet effective solutions for improving our understanding and control of large language models. We showcase how these methods can provide traction on a wide range of safety-relevant problems, including honesty, harmlessness, power-seeking, and more, demonstrating the promise of top-down transparency research. We hope that this work catalyzes further exploration of RepE and fosters advancements in the transparency and safety of AI systems.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Zou, Andy and Phan, Long and Chen, Sarah and Campbell, James and Guo, Phillip and Ren, Richard and Pan, Alexander and Yin, Xuwang and Mazeika, Mantas and Dombrowski, Ann-Kathrin and Goel, Shashwat and Li, Nathaniel and Byun, Michael J. and Wang, Zifan and Mallen, Alex and Basart, Steven and Koyejo, Sanmi and Song, Dawn and Fredrikson, Matt and Kolter, J. Zico and Hendrycks, Dan},
	month = oct,
	year = {2023},
	note = {arXiv:2310.01405 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Computers and Society, Computer Science - Machine Learning},
	annote = {Comment: Code is available at https://github.com/andyzoujm/representation-engineering},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/MU6LDRB5/Zou et al. - 2023 - Representation Engineering A Top-Down Approach to.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/6WJLBJFU/2310.html:text/html},
}

@misc{turner_activation_2023,
	title = {Activation {Addition}: {Steering} {Language} {Models} {Without} {Optimization}},
	shorttitle = {Activation {Addition}},
	url = {http://arxiv.org/abs/2308.10248},
	doi = {10.48550/arXiv.2308.10248},
	abstract = {Reliably controlling the behavior of large language models is a pressing open problem. Existing methods include supervised finetuning, reinforcement learning from human feedback, prompt engineering, and guided decoding. We instead investigate activation engineering: modifying activations at inference time to predictably alter model behavior. In particular, we bias the forward pass with an added 'steering vector' implicitly specified through natural language. Unlike past work which learned these steering vectors, our Activation Addition (ActAdd) method computes them by taking the activation differences that result from pairs of prompts. We demonstrate ActAdd on GPT-2 on OpenWebText and ConceptNet. Our inference-time approach yields control over high-level properties of output and preserves off-target model performance. It involves far less compute and implementation effort than finetuning, allows users to provide natural language specifications, and its overhead scales naturally with model size.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Turner, Alexander Matt and Thiergart, Lisa and Udell, David and Leech, Gavin and Mini, Ulisse and MacDiarmid, Monte},
	month = sep,
	year = {2023},
	note = {arXiv:2308.10248 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Machine Learning},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/M2BJG8CN/Turner et al. - 2023 - Activation Addition Steering Language Models With.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/TSUVSDC6/2308.html:text/html},
}

@misc{hu_lora_2021,
	title = {{LoRA}: {Low}-{Rank} {Adaptation} of {Large} {Language} {Models}},
	shorttitle = {{LoRA}},
	url = {http://arxiv.org/abs/2106.09685},
	doi = {10.48550/arXiv.2106.09685},
	abstract = {An important paradigm of natural language processing consists of large-scale pre-training on general domain data and adaptation to particular tasks or domains. As we pre-train larger models, full fine-tuning, which retrains all model parameters, becomes less feasible. Using GPT-3 175B as an example -- deploying independent instances of fine-tuned models, each with 175B parameters, is prohibitively expensive. We propose Low-Rank Adaptation, or LoRA, which freezes the pre-trained model weights and injects trainable rank decomposition matrices into each layer of the Transformer architecture, greatly reducing the number of trainable parameters for downstream tasks. Compared to GPT-3 175B fine-tuned with Adam, LoRA can reduce the number of trainable parameters by 10,000 times and the GPU memory requirement by 3 times. LoRA performs on-par or better than fine-tuning in model quality on RoBERTa, DeBERTa, GPT-2, and GPT-3, despite having fewer trainable parameters, a higher training throughput, and, unlike adapters, no additional inference latency. We also provide an empirical investigation into rank-deficiency in language model adaptation, which sheds light on the efficacy of LoRA. We release a package that facilitates the integration of LoRA with PyTorch models and provide our implementations and model checkpoints for RoBERTa, DeBERTa, and GPT-2 at https://github.com/microsoft/LoRA.},
	urldate = {2023-10-17},
	publisher = {arXiv},
	author = {Hu, Edward J. and Shen, Yelong and Wallis, Phillip and Allen-Zhu, Zeyuan and Li, Yuanzhi and Wang, Shean and Wang, Lu and Chen, Weizhu},
	month = oct,
	year = {2021},
	note = {arXiv:2106.09685 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
	annote = {Comment: Draft V2 includes better baselines, experiments on GLUE, and more on adapter latency},
	file = {arXiv Fulltext PDF:/Users/joshuaclymer/Zotero/storage/2HK4S8WE/Hu et al. - 2021 - LoRA Low-Rank Adaptation of Large Language Models.pdf:application/pdf;arXiv.org Snapshot:/Users/joshuaclymer/Zotero/storage/CIRH87TA/2106.html:text/html},
}

